Bipartite entanglement of large quantum systems

In this thesis we study the behavior of bipartite entanglement of a large quantum system, by analyzing the distribution of the Schmidt coefficients of the reduced density matrix. Applying the general methods of classical statistical mechanics, we develop a canonical approach for the study of the distribution of these coefficients for a fixed value of the average entanglement. We introduce a partition function depending on a fictitious temperature, which localizes the measure on the set of states with higher and lower entanglement, if compared to typical (random) states with respect to the Haar measure. The purity of one subsystem, which is our entanglement measure/indicator, plays the role of energy in the partition function. This thesis consists of two parts. In the first part, we completely characterize the distribution of the purity and of the eigenvalues for pure states. The global picture unveils several locally stable solutions exchange stabilities, through the presence of first and second order phase transitions. We also detect the presence of metastable states. In the second part, we focus on mixed states. Through the same statistical approach, we determine the exact expression of the first two moments of the local purity and the high temperature expansion of the first moment. We also bridge our problem with the theory of quantum channels, more precisely we exploit the symmetry properties of the twirling transformations in order to compute the exact expression for the first moment of the local purity.

==> concl_copia.tex <==
\chapter*{Conclusions and outlook}\label{conc}
\markboth{Conclusions and outlook}{Conclusions and outlook}
\addcontentsline{toc}{chapter}{Conclusions and outlook}

In this thesis, we have discussed the behavior of bipartite entanglement 
%We have obtained a complete characterization of the statistical features of the bipartite entanglement
of a large quantum system. We have seen that given a bipartite system, the purity of one part can be considered a measure of quantum correlations between the two subsystems only for the case of pure states (that is for isolated quantum systems), while for the more general case of mixed states, this quantity is just a lower bound, and should be substituted with its convex roof. In particular, we have developed a canonical approach for the study of the distribution of the Schmidt coefficients for a fixed value of the average entanglement. We have thus introduced a partition function depending on a fictitious temperature, which localizes the measure on the set of states with higher and lower entanglement with respect to typical (random) states, with respect to the Haar measure. The role of the energy in the partition function is played by our entanglement measure/indicator, the purity of one subsystem.  
%Remember that $\beta$, viewed as a Lagrange multiplier in this statistical mechanical approach, localizes the measure on set of states with a given entanglement (isopurity manifolds \cite{Kus01}).

In the first part of the thesis, we have obtained a complete characterization of the distribution of the purity and of the eigenvalues for the case of pure states. The global picture is interesting as several locally stable solutions exchange stabilities. On the stable branch (solutions of minimal/maximal free energy for positive/negative temperatures) we have unveiled the presence of three main thermodynamic phases for the system, namely the maximally entangled, the typical and the separable phases, separated by critical points. In particular we have enlightened a second order phase transition, associated to a ${\mathbb Z}_2$ symmetry breaking and related to the vanishing of some Schmidt coefficients, followed by a first order phase transition, associated to the evaporation of the largest eigenvalue from the sea of the others.
In the different phases the distribution of the Schmidt coefficients
has very dissimilar profiles. While for large $\beta$ (small purity) the
eigenvalues, all $\Ord{1/N}$, follow the Wigner semicircle law,
they become distributed according to the Wishart law for smaller $\beta$ and larger purity,
across the second order transition. For even smaller (and eventually
negative) values of $\beta$, when purity becomes finite, across the first order phase transition, one eigenvalue evaporates, leaving the sea of the other eigenvalues
$\Ord{1/N}$ and becoming $\Ord{1}$. This is the signature of separability,
this eigenvalue being associated with the emergence of factorization
in the wave function (given the bipartition). This interpretation is
suggestive and hints at a profound modification of the distribution
of the eigenvalues as $\beta$, and therefore the purity, are changed. Summarizing, for the stable solution the purity goes asymptotically from $1/N$ to $1$. This analysis has been achieved by properly scaling $\beta$, in order to yield the correct thermodynamic limit in the partition function. By keeping the same scaling of positive temperatures also for negative $\beta$'s, we have determined a metastable solution for the system. It shows two phase transitions that are both of second order. The first one, called gravity branch, takes place when the Wishart distribution, characterizing typical states, evolves into an asymmetric arcsine distribution. Then, with a second order phase transition, the distribution of the Schmidt coefficients returns symmetric, leading for $\beta\to-\infty$ to maximally entangled states. At the gravity branch we can interpret the expansion of the free energy around the critical temperature as the partition function of random $2$D surfaces, yielding a theory of pure gravity~\cite{Morris91,Di Francesco1993nw}.

In the second part of the thesis we have considered the more involved case of mixed states and through the same statistical approach, we have determined the exact expression of the first two cumulants at $\beta=0$ and the high temperature expansion, for the first moment of the local purity. We have thus generalized the results of \cite{Giraud,Scott2003}, valid for the case of global pure states. Furthermore, we have also introduced an interesting connection between our problem and the theory of quantum channels, more precisely we have exploited the symmetry properties of the twirling transformations~\cite{tw1} in order to compute the exact expression for the first moment of the local purity. 


Our characterization of bipartite entanglement of Haar-distributed states, where the least set of assumptions is made on their generation, can be used in an experiment, \emph{mutatis mutandis}, as a check of the lack of correlations. If one observes that the moments of the purity deviate from the expected values, one could argue for non-randomness (or additional available information) of the states. In turn, our fictitious inverse temperature $\beta$ acquires physical meaning, in that it measures deviations from typicality. This analysis also answers to another, more practical, question: since during the study of some features of entanglement one often relies on numerical simulations, it is important to know to what extent entangled quantum states may be considered  typical~\cite{Zyczkowski98}.

The analysis performed in this thesis for the study of bipartite entanglement of large quantum systems, offers several possible perspectives for future investigation.
From the point of view of quantum information, it would be of great interest to determine the evolution of the entanglement phase
transitions we have studied for the case of pure states, for the more general case of mixed states, when  a new degree of freedom, given by the purity of the global state, is introduced. In this context, another outstanding result would be to understand whether these phase transitions survive even in  the multipartite entanglement scenario \cite{multipartitoClassStat},
if one views the distribution of purity (over all balanced
bipartitions) as a characterization of the global entanglement of
the many-body wave function of quantum systems \cite{mmes}.
%This description of multipartite entanglement displays the symptoms of frustration \cite{frust,frustbis}, catapulting the problem into one of the most fascinating arenas of modern statistical mechanics \cite{parisi}.
\\
Finally, we observe that the phase transitions investigated in this thesis, through a classical statistical mechanics approach are not quantum phase transitions~\cite{Sachdev99}. Nevertheless, entanglement is known to be a good indicator of  quantum phase transitions \cite{osterloh02}, not only for what concerns bipartite entanglement \cite{vidal03,VerstraetePopp2004} but also for the case of multipartite entaglement \cite{costantini2007,xxdiag}. Thus it would be interesting to investigate the link, if any, between these different phase transitions, and therefore apply the techniques shown in this work in order to explore new appealing features of many-body systems, such as spin chains and systems which show a critical behavior. 

We believe that, since the approach followed in this thesis is rooted on the intersection of many aspects of theoretical physics (from classical statistical mechanics, to quantum information, to random matrix theory) it can be regarded as a useful methodological framework for further and even more general topics of investigation. 
%While we were completing this work a paper appeared in which an aspect of this problem is discussed, although with a different emphasis \cite{Majumdar09}. In order to connect our results to those in \cite{Majumdar09}, notice that the probability distribution of the purity $P(u)$  is proportional to the volume of the isopurity manifold and therefore 
%\begin{equation}
%\ln P(u)\simeq N^2 s(u) ,  
%\end{equation}
%where $s$ is the entropy and $N\langle \pi_{AB}\rangle=u$ is the internal energy. See Eq.\ (\ref{eq:1122}).

 



%\rev{The outcome of this statistical approach to bipartite entanglement will be twofold. On the one hand  
%we will distinguish three main entanglement phases (or regions): maximally entangled, typical and separable phase. These regions are
%separated by first and second order phase transitions. On the other hand, by the explicit computation of the entropy of the system, we will evaluate the volume of
%the manifolds in the Hilbert space with constant purity (iso-purity manifolds). The last point enhances the interest in this subject, for more than one reason. First of all, from a philosophical point of view, this answers to the question of determining how probable is finding an entangled state, for a large quantum system. The second reason is more practical: since during the analysis of some features of entanglement one often relies on numerical simulations, it is important to know to what extent entangled quantum states may be considered as typical~\cite{Zyczkowski98}.

%Notice that the phase transitions we will investigate in this thesis, appearing thru a classical statical mechanics approach are not quantum phase transitions. Nevertheless, entanglement is known to be a good indicator of  quantum phases transitions \cite{osterloh02}, not only for what concerns bipartite entanglement \cite{vidal03,VerstraetePopp2004} but also multipartite entaglement \cite{costantini2007,xxdiag}, whose distribution has been characterized by computing the first three cumulants with the same classical statistical approach discussed above \cite{multipartitoClassStat}. Thus it would be interesting to investigate the link, if any, between these different phase transitions.  }
 
 
% **************************************************************************************************************************************************************************************

%\rev{abstract PRA}We study the distribution of the Schmidt coefficients of the reduced density matrix of a quantum system in a pure state.
%By applying general methods of statistical mechanics, we introduce a fictitious temperature and a partition function and
%translate the problem in terms of the distribution of the eigenvalues of random matrices. We investigate the appearance of two phase transitions, one at a positive temperature, associated to very entangled states, and one at a negative temperature, signalling the appearance of a significant factorization in the many-body wave function. We also focus on the presence of metastable states (related to 2-D quantum gravity) and study the finite size corrections to the saddle point solution.



%\rev{ramo stabile e metastable, preso da metast di PRA, fine pag 8}


% In the next section we will show that a first order phase transition occurs at a lower value of $\beta$, namely at $\beta\simeq -2.455/N$ in this scaling (and therefore the exponent $\alpha$ needs to be lowered from 3 to 2 for negative $\beta$). The new stable phase will take over for all negative $\beta$, where $\beta=-\infty$ corresponds to separable states.
%However the metastable branch which emanates from the analytic continuation described here exists for all negative $\beta$ and we can study in more detail the behavior of the eigenvalue density (\ref{eq:phi(x)}) and of its free energy (\ref{eq:freeenergy}).
%The solution is straightforward but lengthy and is given in the following.


%\rev{vecchia intro part1}
%In the first part of this Thesis we intend to characterize the statistical properties of bipartite entanglement for a large quantum system in a pure state. Beside being of interest for applications, this reveals
%an interesting problem in statistical mechanics. It will be tackled by studying a random matrix model that describes the
%distribution of an entanglement measure,
%the purity of one of the two subsystems~\cite{paper1,metastable}. In the
%context of quantum information this technique was already introduced in order to describe the statistics of the eigenvalues of
%the reduced density matrix of a subsystem and extract the first
%moments of some quantities of interest, like the entanglement
%entropy or the purity ~\cite{Lloyd1988,page,Scott2003}. In particular, we will introduce a partition function for the canonical ensemble as a
%function of a fictitious temperature. The purity will play the role of the energy of the system, that is different temperatures will correspond to
%different entanglement.  The outcome of this statistical approach to bipartite entanglement will be twofold. On the one hand  
%we will distinguish three main entanglement phases (or regions): maximally entangled, typical and separable phase. These regions are
%separated by first and second order phase transitions. On the other hand, by the explicit computation of the entropy of the system, we will evaluate the volume of
%the manifolds in the Hilbert space with constant purity (iso-purity manifolds).

%The last point enhances the interest in this subject, for more than one reason. First of all, from a philosophical point of view, this answers to the question of determining how probable is finding an entangled state, for a large quantum system. The second reason is more practical: since during the analysis of some features of entanglement one often relies on numerical simulations, it is important to know to what extent entangled quantum states may be considered as typical~\cite{Zyczkowski98}.

%We will devote the next five chapters of the Thesis to this statistical analysis of bipartite entanglement of pure quantum states. 
%In Chap.~\ref{chap2} we will introduce the notation and set the bases of the statistical mechanics approach to the problem.
%In Chap.~\ref{chap3} we will study the case of positive temperatures, where at very low temperatures we will find very entangled states.
%Negative temperatures will be investigated in Chap.~\ref{chap4} and~\ref{chap5} as we will show that two branches exist, a stable one associated to a partial factorization of the many-body wave function, and a metastable branch which contains the 2D-quantum gravity point. We will also investigate the finite size corrections. Finally  in Chap.~\ref{chap6} we will overview the results of the previous chapters, by reinterpreting them directly from the point of quantum information.

%, and discuss the implications and future perspectives of our results for quantum information.

%In the next part of this Thesis we will move to the case of mixed quantum state. 

%As can be expected, the generalization of this statistical analysis  will not be straightforward, for at least two reasons. First of all, as showed in Chap.~\ref{chap1}, there is not a unique measure of entanglement for arbitrary mixed states. Secondly, since statistical mixtures do not live in a vector Hilbert space, there is not a unique and natural random matrix model for the description of the statistical properties of the system when the restriction of pure states is removed. 


==> first.tex <==
\setlength{\voffset}{-1.cm}
\begin{center}
  %\begin{titlepage} 
  \begin{center}
    \begin{figure}
     \begin{center}
    \includegraphics[width=3.5cm]{barilogo}
      \end{center} 
    \end{figure}
		    {\Large {\bf UNIVERSIT\`A DEGLI STUDI DI BARI \\  \vskip 1.5 mm ALDO MORO}} \\  \vskip 2mm
		    {{\bf DIPARTIMENTO DI FISICA  ``MICHELANGELO MERLIN"}} \\ \vskip 1mm
		    		     {{\bf DOTTORATO DI RICERCA IN FISICA - Ciclo XXIII}}
				\vskip 1.5 mm     Settore Scientifico Disciplinare FIS/02
		     \rule{380pt}{1pt} \end{center}
 
   
  \vspace{3cm}
 % \huge{\sc{Ph.D. Thesis}}
  %\vspace{2.5cm}
   \setlength{\textwidth}{12cm}
  \begin{minipage}{\textwidth}
   \begin{center}
       {\Large {\bf BIPARTITE ENTANGLEMENT     \\ OF LARGE QUANTUM SYSTEMS \\}}
%     \vspace{2 mm}
%    {\bf FROM LARGE TO SMALL QUANTUM SYSTEMS}
   \end{center}
  \end{minipage}
\end{center}
      \vspace{1.5cm}
  \begin{center}    
 \Large {\bf Antonella De Pasquale}
  \end{center}    

  \vskip 2.5cm
  \begin{center}
\large{Final Exam, 2011}
\end{center}
  \vspace{8em}
  \nopagebreak[4]
  %\end{titlepage}

\newpage
\thispagestyle{empty}


==> firstCONTOM.tex <==
\setlength{\voffset}{-1.cm}
\begin{center}
  %\begin{titlepage} 
  \begin{center}
    \begin{figure}
     \begin{center}
    \includegraphics[width=3.5cm]{barilogo}
      \end{center} 
    \end{figure}
		    {\Large {\bf UNIVERSIT\`A DEGLI STUDI DI BARI \\  \vskip 1.5 mm ALDO MORO}} \\  \vskip 2mm
		    {{\bf DIPARTIMENTO DI FISICA  ``MICHELANGELO MERLIN"}} \\ \vskip 1mm
		    		     {{\bf DOTTORATO DI RICERCA IN FISICA - Ciclo XXIII}}
		     \rule{380pt}{1pt} \end{center}
 
   
  \vspace{2.5cm}
 % \huge{\sc{Ph.D. Thesis}}
  %\vspace{2.5cm}
   \setlength{\textwidth}{12cm}
  \begin{minipage}{\textwidth}
   \begin{center}
       {\Large {\bf ASPECTS OF \\ BIPARTITE ENTANGLEMENT     \\ AND TOMOGRAPHY \\}}
     \vspace{2 mm}
    {\bf FROM LARGE TO SMALL QUANTUM SYSTEMS}
   \end{center}
  \end{minipage}
\end{center}
      \vspace{2.3cm}
\noindent{\bf Dottoranda}: \\{\large\sc Antonella De Pasquale}

\begin{flushright}
{\bf Supervisori}: \\
{\large\sc Prof.~Paolo~Facchi\\
Prof.~Saverio~Pascazio}
\end{flushright}

  \vskip 1.8cm
  \begin{center}
\large{December, 2010}
\end{center}
  \vspace{8em}
  \nopagebreak[4]
  %\end{titlepage}

\newpage
\thispagestyle{empty}


==> firstcopia.tex <==
\setlength{\voffset}{-0.cm}
\begin{center}
  %\begin{titlepage} 
  \begin{center}
    \begin{figure}
     \begin{center}
    \includegraphics[width=3.5cm]{barilogo}
      \end{center} 
    \end{figure}
		    {\Large {\bf UNIVERSIT\`A DEGLI STUDI DI BARI \\  \vskip 1.5 mm ALDO MORO}} \\  \vskip 2mm
		    {{\bf DIPARTIMENTO INTERATENEO DI FISICA   \\  \vskip 1mm``MICHELANGELO MERLIN"}} \\ \vskip 1mm
		    		     {{\bf DOTTORATO DI RICERCA IN FISICA - Ciclo XXIII}} \\ \vskip 1mm  {{ \bf Settore Scientifico Disciplinare FIS/02}}
				     
		     \rule{380pt}{1pt} \end{center}
 
   
  \vspace{1cm}
 % \huge{\sc{Ph.D. Thesis}}
  %\vspace{2.5cm}
   \setlength{\textwidth}{12cm}
  \begin{minipage}{\textwidth}
   \begin{center}
       {\Large {\bf BIPARTITE ENTANGLEMENT     \\ OF LARGE QUANTUM SYSTEMS \\}}
%     \vspace{2 mm}
%    {\bf FROM LARGE TO SMALL QUANTUM SYSTEMS}
   \end{center}
  \end{minipage}
\end{center}
      \vspace{1.cm}
\noindent{\bf Dottoranda}: \\{\large\sc Antonella De Pasquale}

\vspace{0.8cm}
\begin{flushright}
{\bf Coordinatore}: \\
{\large\sc Ch.mo Prof.~Francesco~Romano}
\end{flushright}


 \vspace{0.6cm}
\noindent{\bf Supervisori}: \\{\large\sc Ch.mo Prof. Paolo Facchi  \\  \vskip 0.7cm \noindent Ch.mo Prof. Saverio Pascazio}

  \vskip 2.4cm
  \begin{center}
\large{ESAME FINALE 2011}
\end{center}
  \vspace{8em}
  \nopagebreak[4]
  %\end{titlepage}

\newpage
\thispagestyle{empty}


==> introPapers.tex <==


\newpage
\thispagestyle{empty}
\mbox{}

\chapter*{}


During my three years as a Ph.D. candidate I worked on several topics of
theoretical physics, other than bipartite entanglement and random matrices. These activities
focused on spin chains, quantum phase transitions, quantum tomography and open quantum systems. In the following I include some papers that I published during
my Ph.D.  studies and that have not been discussed in the Thesis for lack of
space.
